Optimization of Quadratic Constraints by Decoded Quantum Interferometry

A recent paper by Jordan et al. introduced Decoded Quantum Interferometry (DQI), a novel quantum algorithm that uses the quantum Fourier transform to reduce linear optimization problems -- max-XORSAT and max-LINSAT -- to decoding problems. In this paper, we extend DQI to optimization problems involving quadratic constraints, which we call max-QUADSAT. Leveraging a connection to quadratic Gauss sums, we give an efficient algorithm to prepare the DQI state for max-QUADSAT (DISCLAIMER: A mistake was found in one of the algorithm's steps, which invalidates this result unless a fix is found). To demonstrate that our algorithm achieves a quantum advantage, we introduce the Quadratic Optimal Polynomial Intersection (quadratic-OPI) problem, a restricted variant of OPI for which, to our knowledge, the standard DQI framework offers no algorithmic speedup. We show that quadratic-OPI is an instance of max-QUADSAT and use our algorithm to optimize it. Lastly, we present a new generalized proof of the "semicircle law" for the fraction of satisfied constraints, generalizing it to any DQI state of problems where the distribution of the number of satisfied constraints for a random assignment is sufficiently close to a binomial distribution. This condition holds exactly for the DQI state of max-LINSAT, and approximately holds in the max-QUADSAT case, with the approximation becoming exponentially better as the problem size increases. This establishes performance guarantees for our algorithm.

==> optimal_expected_fraction_satisfied.tex <==
\section{Optimal Asymptotic Expected Fraction of Satisfied Constraints}
\begin{wiparea}
I'm assuming there are only quadratic constraints and that the matrices commute here.

\begin{lemma}
    TODO: Add equivalent lemma to Lemma 9.1 in \cite{og_dqi}. That is, for our modified quadratic code, $\big< \tilde{P} (f) \big| \tilde{P}(f) \big> = \left|\middle| \mathbf{w} \middle|\right|$, where $\mathbf{w}$ is the vector of the elementary symmetric polynomial weights $w_1, \dots, w_\ell$
\end{lemma}

Let $F_i$ be the preimage of $+1$ for the constraint function $f_i$. The number of constraints satisfied by $\x \in \F_p^n$ is
\begin{equation} \label{eq:s_num_of_sat_constraints}
    s(\x) = \sum_{i=1}^m \mathbbm{1}_{F_i}(\mathbf{b}_i^T \x + \x^T C_i \x)
\end{equation}
Where $\mathbbm{1}$ is the \textit{indicator function}, defined for a set $A$ as
\begin{equation}
    \mathbbm{1}_A(x) = \begin{cases}
        1 & \text{if $x \in A$} \\
        0 & \text{if $x \notin A$}
    \end{cases}
\end{equation}
We can use the well-known properties of sums of roots of unity to write for $v, x \in \F_p$
\begin{equation}
    \mathbbm{1}_{\set{v}}(x) = \frac{1}{p}\sum_{a \in \F_p} \omega_p^{a(x-v)}
\end{equation}
Hence, by writing $F_i$ in terms of its elements
\[
    \mathbbm{1}_{F_i}(x)
    = \sum_{v \in F_i} \mathbbm{1}_{\set{v}}(x)
    = \frac{1}{p} \sum_{v \in F_i} \sum_{a \in \F_p} \omega_p^{a(x-v)}
\]
Plugging that into \autoref{eq:s_num_of_sat_constraints} yields
\begin{equation}
    s(\x)
    =
    \frac{1}{p} \sum_{i=1}^m \sum_{v \in F_i} \sum_{a \in \F_p}
    \omega_p^{a(\mathbf{b}_i^T\x + \x^TC_i\x-v)}
\end{equation}
We are interested in the expected number of satisfied constraints for the DQI state defined in \autoref{def:dqi_state_max_quadsat}. To do so, we will define the operator
\begin{equation}
\begin{aligned}
    S_f &=
            \sum_{\x \in \F_p^n}
            s(\x) \left| \x \right> \left< \x \right|
     \\ &= \frac{1}{p}
            \sum_{\x \in \F_p^n} 
            \sum_{i=1}^m
            \sum_{v \in F_i}
            \sum_{a \in \F_p}
            \omega_p^{a(\mathbf{b}_i^T\x + \x^TC_i\x-v)}
        \left| \x \right> \left< \x \right|
     \\ &= \frac{1}{p}
            \sum_{i=1}^m
            \sum_{v \in F_i}
            \sum_{a \in \F_p}
            \omega_p^{-av}
            \sum_{\x \in \F_p^n} 
            \omega_p^{a(\mathbf{b}_i^T\x + \x^TC_i\x)}
        \left| \x \right> \left< \x \right|
\end{aligned}
\end{equation}

\subsection{Attempt: simpler case where the matrices commute and no linear}
Now we can write the operator $S_f$ as
\begin{equation}
\begin{aligned}
    S_f &= \frac{1}{p}
            \sum_{i=1}^m
            \sum_{v \in F_i}
            \sum_{a \in \F_p}
            \omega_p^{-av}
            \sum_{\x \in \F_p^n} 
            \omega_p^{a(\x^TC_i\x)}
        \left| \x \right> \left< \x \right|
     \\ &= \frac{1}{p}
            \sum_{i=1}^m
            \sum_{v \in F_i}
            \sum_{a \in \F_p}
            \omega_p^{-av}
            \sum_{\x \in \F_p^n} 
            \omega_p^{a(\x^TD_i\x)}
        \left| O\x \right> \left< O\x \right|
\end{aligned}
\end{equation}
Let $U_O$ denote the unitary operator $U_O \left| \x \right> = \left| O \x \right>$, from now on we will look at the operator $U_O^\dagger S_f U_O$ instead
\begin{equation}
\begin{aligned}
    U_O^\dagger S_fU_O &= \frac{1}{p}
            \sum_{i=1}^m
            \sum_{v \in F_i}
            \sum_{a \in \F_p}
            \omega_p^{-av}
            \sum_{\x \in \F_p^n} 
            \omega_p^{a(\x^TD_i\x)}
        \left| \x \right> \left< \x \right|
     \\ &= \frac{1}{p}
            \sum_{i=1}^m
            \sum_{v \in F_i}
            \sum_{a \in \F_p}
            \omega_p^{-av}
            \prod_{j=1}^n
            \sum_{x_j \in \F_p} 
            \omega_p^{a D_{ij} x_j^2}
        \left| x_j \right> \left< x_j \right|
\end{aligned}
\end{equation}
This leads us to the following definition, inspired by the clock and shift operators (TODO: Add analog of shift operator)
\begin{definition}[clock and shift operators] \label{def:clock_shift_operators}
    The clock operator is defined as
    \begin{equation}
        Z = \sum_{b \in \F_p} \omega_p^{b} \left| b \right> \left< b \right|
    \end{equation}
    And the shift operator is defined as
    \begin{equation}
        X = \sum_{x \in \F_p} \left| x+1 \right> \left< x \right|
    \end{equation}
\end{definition}

\begin{definition}[quadratic clock operator] \label{def:quadratic_clock_operator}
    We define the quadratic clock operator as
    \begin{equation}
        Z_2 = \sum_{b \in \F_p} \omega_p^{b^2} \left| b \right> \left< b \right|
    \end{equation}
\end{definition}
\begin{lemma}[clock is shift in Fourier basis]
    Let $F = \sum_{x,y \in \F_p} \omega_p^{x y} \left| x \right> \left< y \right|$ be the quantum Fourier transform operator, and let $Z = \sum_{b \in \F_p} \omega_p^{b} \left| b \right> \left< b \right|$ be the clock operator as defined in \autoref{def:clock_shift_operators}, then the following relation holds
    \begin{equation}
        F Z F^\dagger = X^{-1}
    \end{equation}
\end{lemma}
\begin{proof}
    \begin{equation}
    \begin{aligned}
        F Z F^\dagger
        &=
        \sum_{x,y,x',y',b \in \F_p}
        \omega_p^{xy - x'y' + b} 
            \left| x \right>
            \underbrace{\left< y \middle| b \right>}_{\delta_{y,b}}
            \underbrace{\left< b \middle| y' \right>}_{\delta_{b, y'}}
            \left< x' \right|
        \\ &=
        \sum_{x,x' \in \F_p}
        \underbrace{
            \sum_{b \in \F_p}
            \omega_p^{\left(x - x' + 1\right) b}
        }_{\delta_{x, x'-1}}
            \left| x \right>
            \left< x' \right|
        \\ &=
        \sum_{x \in \F_p}
            \left| x - 1 \right>
            \left< x \right|
    \end{aligned}
    \end{equation}
\end{proof}
\begin{lemma}[quadratic clock is quadratic shift in Fourier basis TODO]
    Let $F$ be the quantum Fourier transform operator, and let $Z_2$ be the quadratic clock operator \autoref{def:quadratic_clock_operator}, then
    \begin{equation}
        F Z_2 F^\dagger
        =
        ????
    \end{equation}
\end{lemma}
\begin{proof}
    \begin{equation}
    \begin{aligned}
        F Z_2 F^\dagger
        &=
        \sum_{x,x' \in \F_p}
            \sum_{b \in \F_p}
            \omega_p^{\left(x - x' + b\right) b}
            \left| x \right>
            \left< x' \right|
        \\ &\xeq{b \to b - (x-x')}
        \sum_{x,x' \in \F_p}
            \sum_{b \in \F_p}
            \omega_p^{\left(\frac{1}{2}(x - x') + b\right) \left( b - \frac{1}{2}(x - x')\right)}
            \left| x \right>
            \left< x' \right|
        \\ &=
        \sum_{x,x' \in \F_p}
            \omega_p^{-\frac{1}{4} (x-x')^2}
            \underbrace{
                \sum_{b \in \F_p}
                \omega_p^{b^2}
            }_{g(1; p)}
            \left| x \right>
            \left< x' \right|
        \\ &=
        g(1; p)
        \sum_{x,x' \in \F_p}
            \omega_p^{-\frac{1}{4} (x-x')^2}
            \left| x \right>
            \left< x' \right|
    \end{aligned}
    \end{equation}
\end{proof}
We note that
\[
    U_O^\dagger S_f U_O = 
    \frac{1}{p}
    \sum_{i=1}^m
    \sum_{v \in F_i}
    \sum_{a \in \F_p}
    \omega_p^{-av}
    \prod_{j=1}^n
    Z_2^{a D_{ij}}
\]


\[
\begin{aligned}
    \left< P(f) \right| S_f \left| P(f) \right>
\end{aligned}
\]

\[
\begin{aligned}
    \left< s^{(m, \ell)} \right>
    =
    \frac{1}{p}
    \sum_{k_1, k_2 = 0}^\ell
    \frac{w_{k_1}^* w_{k_2}}{\sqrt{\binom{m}{k_1} \binom{m}{k_2}}}
    \sum_{\substack{\y_1, \y_2 \in \F_p^n \\ |\y_1| = k_1 \\ | \y_2 | = k_2}}
    \sum_{\z_1, \z_2 \in \F_p^n}
    \alpha_{\y_1} \alpha_{\y_2}
    \omega_p^{-\frac{1}{4} \z_1^T ( C \cdot \y_1 )^{-1} \z_1 + \frac{1}{4} \z_2^T ( C \cdot \y_2 )^{-1} \z_2}
    % Q^*(\z_1, \y_1)
    % Q(\z_2, \y_2)
    \tilde{g}^*(\y_1) \tilde{g}(\y_2)
    \\
    \sum_{i=1}^m
    \sum_{v \in F_i}
    \sum_{a \in \F_p}
    \omega_p^{-av}
    \left< \z_1 \right|
    \prod_{j=1}^n X_{j,2}^{aD_{ij}}
    \left| \z_2 \right>
\end{aligned}
\]
TODO: What happened to the product over $j$?
\[
\begin{aligned}
    =
    g(1;p)
    \frac{1}{p}
    \sum_{k_1, k_2 = 0}^\ell
    \frac{w_{k_1}^* w_{k_2}}{\sqrt{\binom{m}{k_1} \binom{m}{k_2}}}
    \sum_{\substack{\y_1, \y_2 \in \F_p^n \\ |\y_1| = k_1 \\ | \y_2 | = k_2}}
    \sum_{\z_1, \z_2 \in \F_p^n}
    \alpha_{\y_1} \alpha_{\y_2}
    \omega_p^{-\frac{1}{4} \z_1^T ( C \cdot \y_1 )^{-1} \z_1 + \frac{1}{4} \z_2^T ( C \cdot \y_2 )^{-1} \z_2}
    % Q^*(\z_1, \y_1)
    % Q(\z_2, \y_2)
    \tilde{g}^*(\y_1) \tilde{g}(\y_2)
    \\
    \sum_{i=1}^m
    \sum_{v \in F_i}
    \underbrace{
        \sum_{a \in \F_p}
        \omega_p^{-av}
        \omega_p^{-\frac{1}{4} a D_{ij} (\z_2 - \z_1)^2}
    }_{v = -\frac{1}{4}D_{ij} (\z_2 - \z_2)^2}
\end{aligned}
\]
\[
\begin{aligned}
    =
    g(1;p)
    \frac{1}{p}
    \sum_{k_1, k_2 = 0}^\ell
    \frac{w_{k_1}^* w_{k_2}}{\sqrt{\binom{m}{k_1} \binom{m}{k_2}}}
    \sum_{\substack{\y_1, \y_2 \in \F_p^n \\ |\y_1| = k_1 \\ | \y_2 | = k_2}}
    \sum_{\z_1, \z_2 \in \F_p^n}
    \alpha_{\y_1} \alpha_{\y_2}
    \omega_p^{-\frac{1}{4} \z_1^T ( C \cdot \y_1 )^{-1} \z_1 + \frac{1}{4} \z_2^T ( C \cdot \y_2 )^{-1} \z_2}
    % Q^*(\z_1, \y_1)
    % Q(\z_2, \y_2)
    \tilde{g}^*(\y_1) \tilde{g}(\y_2)
    \\
    \sum_{i=1}^m
    \underbrace{
        \sum_{v \in F_i}
        p\delta_{v, -\frac{1}{4}D_{ij} (\z_2 - \z_2)^2}
    }_{p\mathbbm{1}_{F_i}(-\frac{1}{4}D_{ij} (\z_2 - \z_2)^2)}
\end{aligned}
\]


% TODO: Maybe define and use a "quadratic Fourier transform" everywhere

\end{wiparea}

\subsection{Attempt: Quadratic Fourier Transform}

\begin{wiparea}
    TODO
    \[
    \left| x \right>
    \to
    \sum_{y \in \F_p} \omega_p^{x y^2} \left| y \right>
    \]
\end{wiparea}

